Order-forcing in Neural Codes

Convex neural codes are subsets of the Boolean lattice that record the intersection patterns of convex sets in Euclidean space. Much work in recent years has focused on finding combinatorial criteria on codes that can be used to classify whether or not a code is convex. In this paper we introduce order-forcing, a combinatorial tool which recognizes when certain regions in a realization of a code must appear along a line segment between other regions. We use order-forcing to construct novel examples of non-convex codes, and to expand existing families of examples. We also construct a family of codes which shows that a dimension bound of Cruz, Giusti, Itskov, and Kronholm (referred to as monotonicity of open convexity) is tight in all dimensions.

==> arxiv version/shortcuts.tex <==
%%%
% This is a whole bunch of macros/commands/shortcuts I use all the time, so I'm putting them in a single file to be input into anything I'm working on.
% Created August 3, 2015 by Alex Kunin
% Update Feb 19, 2018: Added \rp, \op, \rpf, \opf for real projective and "oriented projective" space, with "f" for excluding the point (0:1). Also made comment section headers stand out more.
% Update Mar 14, 2018: Added environments and references for those environments
% Apr 27, 2018: A few more operators and fixed some greek letters
% May 18, 2018: Added \sK for sans-serif K
% Aug 17, 2018: Added \tr for trace, \argmin for argmin
% Dec 6, 2018: Added some category theory stuff for trunk morphisms
% Nov 2019: Removed \sK and \sF, added \sf* for mathsf characters
% Nov 22, 2019: Added some overrides to package cleveref
% Dec 16, 2019: Added \OMRing for the essential image of the functor OM -> Ring
%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% ENVIRONMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%% A BETTER WAY: package cleveref handles all of this for you, as well as allowing references to multiple things (e.g. \cref{thm1,thm2} will be typeset as "Theorems 1 and 2"). So, all we need to do is override how it displays things when the default is buns.
% Syntax is \crefname{type}{singular}{plural} to change lower-case (mid-sentence) references.
% \Crefname{type}{singular}{plural} changes capitalized references (e.g. start of sentence). Since we use option [capitalize], we don't need to bother with \Crefname at the moment.
\crefname{figure}{Figure}{Figures}
\crefname{prop}{Proposition}{Propositions}

\theoremstyle{definition} 


\newtheorem{bigthm}{Theorem}   % Numbered separately, as A, B, etc.
\newtheorem{thm}{Theorem}[section]   % Numbered within each section
\newtheorem{cor}[thm]{Corollary}     % Numbered along with thm
\newtheorem{lem}[thm]{Lemma}         % Numbered along with thm
\newtheorem{prop}[thm]{Proposition}  % Numbered along with thm
\newtheorem{obs}[thm]{Observation}  % Numbered along with thm
\newtheorem{const}[thm]{Construction}  % Numbered along with thm

\theoremstyle{definition} 
\newtheorem{defn}[thm]{Definition}   % Numbered along with thm
\newtheorem{conj}[thm]{Conjecture}        % Numbered along with thm
\newtheorem*{conj*}{Conjecture}        % Numbered along with thm
\newtheorem{ex}[thm]{Example}        % Numbered along with thm
\newtheorem{exercise}[thm]{Exercise}        % Numbered along with thm
\newtheorem{defprop}[thm]{Definition/Proposition}  % Numbered along with thm

\newtheorem{rmk}[thm]{Remark}
\newtheorem{question}[thm]{Question}
\newtheorem{prob}[thm]{Problem}
\newtheorem{notn}[thm]{Notation}

%%%%% REFERENCES TO ENVIRONMENTS
\newcommand{\refS}[1]{Section~\ref{S:#1}}
\newcommand{\refA}[1]{Appendix~\ref{S:#1}}

\newcommand{\refT}[1]{Theorem~\ref{T:#1}}
\newcommand{\refC}[1]{Corollary~\ref{C:#1}}
\newcommand{\refL}[1]{Lemma~\ref{L:#1}}
\newcommand{\refP}[1]{Proposition~\ref{P:#1}}
\newcommand{\refD}[1]{Definition~\ref{D:#1}}
\newcommand{\refCn}[1]{Conjecture~\ref{Cn:#1}}
\newcommand{\refEx}[1]{Example~\ref{Ex:#1}}
\newcommand{\refR}[1]{Remark~\ref{R:#1}}
\newcommand{\refQ}[1]{Question~\ref{Q:#1}}
\newcommand{\refN}[1]{Notation~\ref{N:#1}}

%\newcommand{\refEq}[1]{Equation~\ref{eq:#1}}
\newcommand{\refEq}[1]{\eqref{eq:#1}}
\newcommand{\refF}[1]{Figure~\ref{F:#1}}
\newcommand{\refTab}[1]{Table~\ref{Tab:#1}}

\newcommand{\refCo}[1]{Construction~\ref{Co:#1}}
\newcommand{\refAlg}[1]{Algorithm~\ref{Alg:#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% OPERATORS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\aut}{Aut}
\DeclareMathOperator*{\inn}{Inn}
\DeclareMathOperator{\ch}{char}
\DeclareMathOperator{\syl}{Syl}
\DeclareMathOperator{\rad}{rad}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\lc}{lc}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\gal}{Gal}
\DeclareMathOperator{\lcm}{lcm}
\DeclareMathOperator{\mult}{mult}
\DeclareMathOperator{\mor}{Mor}
\DeclareMathOperator{\mat}{Mat}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\spec}{Sp}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\wt}{wt}
\DeclareMathOperator{\code}{code}
\DeclareMathOperator{\rel}{rel}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\tor}{Tor}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\nerve}{nerve}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\inte}{int}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\link}{link}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\oc}{oc}

%%% Code and OM operations
\DeclareMathOperator{\tk}{Tk}
\DeclareMathOperator{\trk}{Trk}
\DeclareMathOperator{\rt}{Rt}
\DeclareMathOperator{\st}{star}

\DeclareMathOperator{\odim}{odim}
\DeclareMathOperator{\cdim}{cdim}

\DeclareMathOperator{\TR}{TR}
\DeclareMathOperator{\gens}{gens}
\DeclareMathOperator{\core}{core}
\DeclareMathOperator{\conv}{conv}


%%% Categories
\DeclareMathOperator{\Code}{\mathbf{Code}}
\DeclareMathOperator{\OMlong}{\mathbf{OrientedMatroid}}
\DeclareMathOperator{\OM}{\mathbf{OM}}
\DeclareMathOperator{\OMatroid}{\mathbf{OM}}
\DeclareMathOperator{\COMlong}{\mathbf{ConditionalOrientedMatroid}}
\DeclareMathOperator{\COM}{\mathbf{COM}}
\DeclareMathOperator{\AOMlong}{\mathbf{AffineOrientedMatroid}}
\DeclareMathOperator{\AOM}{\mathbf{AOM}}
\DeclareMathOperator{\NRing}{\mathbf{NRing}}
\DeclareMathOperator{\Ring}{\mathbf{Ring}}
\DeclareMathOperator{\OMRing}{\mathbf{OMRing}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% COMMON SETS AND SUCH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Misc notation I use a lot
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% projective spaces of sorts
\def\rp{\mathbb{R}P}
\def\rpf{\mathbb{R}P_{fin}}
\def\op{\mathbb{R}O}
\def\opf{\mathbb{R}O_{fin}}

%%% the polar complex of a code
\def\bd{\Gamma}

%%% Loops in matroids
\newcommand{\lop}{\circ}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Blackboard bold letters - some may be overwritten by greek letters!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\A{\mathbb A}
\def\B{\mathbb B}
\def\C{\mathbb C}
\def\D{\mathbb D}
\def\E{\mathbb E}
\def\F{\mathbb F}
\def\G{\mathbb G}
\def\H{\mathbb H}
\def\I{\mathbb I}
\def\J{\mathbb J}
\def\K{\mathbb K}
\def\L{\mathbb L}
\def\M{\mathbb M}
\def\N{\mathbb N}
\def\O{\mathbb O}
\def\P{\mathbb P}
\def\Q{\mathbb Q}
\def\R{\mathbb R}
\def\S{\mathbb S}
\def\T{\mathbb T}
\def\U{\mathbb U}
\def\V{\mathbb V}
\def\W{\mathbb W}
\def\X{\mathbb X}
\def\Y{\mathbb Y}
\def\Z{\mathbb Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Mathcal Letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cA{\mathcal A}
\def\cB{\mathcal B}
\def\cC{\mathcal C}
\def\cD{\mathcal D}
\def\cE{\mathcal E}
\def\cF{\mathcal F}
\def\cG{\mathcal G}
\def\cH{\mathcal H}
\def\cI{\mathcal I}
\def\cJ{\mathcal J}
\def\cK{\mathcal K}
\def\cL{\mathcal L}
\def\cM{\mathcal M}
\def\cN{\mathcal N}
\def\cO{\mathcal O}
\def\cP{\mathcal P}
\def\cQ{\mathcal Q}
\def\cR{\mathcal R}
\def\cS{\mathcal S}
\def\cT{\mathcal T}
\def\cU{\mathcal U}
\def\cV{\mathcal V}
\def\cW{\mathcal W}
\def\cX{\mathcal X}
\def\cY{\mathcal Y}
\def\cZ{\mathcal Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Fancy letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\scA{\mathscr A}
\def\scB{\mathscr B}
\def\scC{\mathscr C}
\def\scD{\mathscr D}
\def\scE{\mathscr E}
\def\scF{\mathscr F}
\def\scG{\mathscr G}
\def\scH{\mathscr H}
\def\scI{\mathscr I}
\def\scJ{\mathscr J}
\def\scK{\mathscr K}
\def\scL{\mathscr L}
\def\scM{\mathscr M}
\def\scN{\mathscr N}
\def\scO{\mathscr O}
\def\scP{\mathscr P}
\def\scQ{\mathscr Q}
\def\scR{\mathscr R}
\def\scS{\mathscr S}
\def\scT{\mathscr T}
\def\scU{\mathscr U}
\def\scV{\mathscr V}
\def\scW{\mathscr W}
\def\scX{\mathscr X}
\def\scY{\mathscr Y}
\def\scZ{\mathscr Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Frak - uppercase
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\fA{\mathfrak A}
\def\fB{\mathfrak B}
\def\fC{\mathfrak C}
\def\fD{\mathfrak D}
\def\fE{\mathfrak E}
\def\fF{\mathfrak F}
\def\fG{\mathfrak G}
\def\fH{\mathfrak H}
\def\fI{\mathfrak I}
\def\fJ{\mathfrak J}
\def\fK{\mathfrak K}
\def\fL{\mathfrak L}
\def\fM{\mathfrak M}
\def\fN{\mathfrak N}
\def\fO{\mathfrak O}
\def\fP{\mathfrak P}
\def\fQ{\mathfrak Q}
\def\fR{\mathfrak R}
\def\fS{\mathfrak S}
\def\fT{\mathfrak T}
\def\fU{\mathfrak U}
\def\fV{\mathfrak V}
\def\fW{\mathfrak W}
\def\fX{\mathfrak X}
\def\fY{\mathfrak Y}
\def\fZ{\mathfrak Z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Frak - lowercase
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\fa{\mathfrak a}
\def\fb{\mathfrak b}
\def\fc{\mathfrak c}
\def\fd{\mathfrak d}
\def\fe{\mathfrak e}
\def\ff{\mathfrak f}
\def\fg{\mathfrak g}
\def\fh{\mathfrak h}
\def\fraki{\mathfrak i}
\def\fj{\mathfrak j}
\def\fk{\mathfrak k}
\def\fl{\mathfrak l}
\def\fm{\mathfrak m}
\def\fn{\mathfrak n}
\def\fo{\mathfrak o}
\def\fp{\mathfrak p}
\def\fq{\mathfrak q}
\def\fr{\mathfrak r}
\def\fs{\mathfrak s}
\def\ft{\mathfrak t}
\def\fu{\mathfrak u}
\def\fv{\mathfrak v}
\def\fw{\mathfrak w}
\def\fx{\mathfrak x}
\def\fy{\mathfrak y}
\def\fz{\mathfrak z}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Sans Serif
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\sfD{\mathsf{D}}
\def\sfF{\mathsf{F}}
\def\sfI{\mathsf{I}}
\def\sfK{\mathsf{K}}
\def\sfL{\mathsf{L}}
\def\sfP{\mathsf{P}}
\def\sfR{\mathsf{R}}
\def\sfS{\mathsf{S}}
\def\sfT{\mathsf{T}}
\def\sfW{\mathsf{W}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% GREEK LETTERS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\a{\alpha}
\def\b{\beta}
\def\g{\gamma}
\def\d{\delta}
\def\D{\Delta}
\def\e{\varepsilon}
\def\G{\Gamma}
\def\i{\iota}
\def\phum{\varphi}
\def\L{\Lambda}
\def\l{\lambda}
\def\m{\mu}
\def\n{\nu}
\def\o{\omega}
\def\O{\Omega}
\def\p{\pi}
\def\P{\Pi}
\def\r{\rho}
\def\s{\sigma}
\def\t{\tau}
\def\th{\theta}
\def\x{\chi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% USEFUL SHORTCUTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\inv{^{-1}}
\def\Sum{\sum_{n=0}^\infty}
\def\sm{\setminus}
\def\sd{\triangle}
\def\br{\overline}
\def\dd{\partial}
\def\od{:=}

\newcommand{\ang}[1]{\left\langle #1\right\rangle}	%put angle brackets around something
%\newcommand{\dang}[1]{\left\langle #1 \right\rangle}	%put angle brackets around something, allowing for fractions/etc. in displaystyle
\newcommand{\flr}[1]{\left\lfloor #1 \right\rfloor} %put floor brackets around something
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\renewcommand{\emptyset}{\varnothing}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% fancy arrows
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\from{\leftarrow}
\def\into{\hookrightarrow}
\def\otni{\hookleftarrow}
\def\onto{\twoheadrightarrow}
\def\otno{\twoheadleftarrow}
\def\inonto{\hookrightarrow \hspace{-8pt} \rightarrow}
\def\conto{\longrightarrow} %for things converging to other things.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Overlined Numerals
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\1{\overline{1}}
\def\2{\overline{2}}
\def\3{\overline{3}}
\def\4{\overline{4}}
\def\5{\overline{5}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Bold Letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}

\def\id{\operatorname{id}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Underlined Letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\uf{\underline{f}}
\def\uE{\underline{E}}
\def\uS{\underline{S}}



